PAGS: Autofocusing Photoacoustic Tomography via Speed-of-Sound-Adaptive Gaussian Splatting

Photoacoustic computed tomography (PACT) combines optical absorption contrast with acoustic detection for high-resolution deep-tissue imaging. A persistent challenge is that unknown speed-of-sound (SoS) heterogeneity changes acoustic time-of-flight, causing defocusing artifacts when reconstruction assumes a uniform SoS. Existing SoS-adaptive methods either rely on calibrated acoustic priors or optimize dense physical medium models, which becomes expensive and difficult to scale in 3D. We propose PAGS, a differentiable framework for blind autofocusing PACT via speed-of-sound-adaptive Gaussian splatting. PAGS represents the initial pressure field with sparse Gaussian photoacoustic (PA) sources and replaces explicit medium recovery with a compact anisotropic path-averaged SoS (ASoS) field parameterized by spherical harmonic probes. This latent propagation field directly controls source-to-transducer arrival-time alignment, while an analytic Gaussian acoustic projection maps the source representation to transducer signals efficiently. The resulting closed-loop signal-domain optimization jointly updates the Gaussian PA source parameters and the ASoS field from measured data, without calibrated SoS priors. Experiments on simulated and physical phantom data demonstrate improved reconstruction sharpness under heterogeneous acoustic media, robustness to sparse-view sampling, and computational benefits from the analytic Gaussian projection.

==> tex/exp_old.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup and Implementation Details}
\label{subsec:exp_setup}

\textbf{Datasets.} To comprehensively evaluate our proposed method, we conducted experiments on both simulated and real-world physical phantoms:
\begin{itemize}
    \item \textit{In Silico Data:} %%% 填写仿真参数，例如：We simulated a complex vascular network using k-Wave with an underlying dual-SoS distribution (e.g., 1500 m/s for background and 1580 m/s for specific regions)... %%%
    \item \textit{Physical Phantoms:} %%% 填写你们搭建的真实 PACT 系统参数，以及 phantom 的材质和预期的声速分层情况。强调它具有明显的异质性... %%%
\end{itemize}

\textbf{Baselines.} We compared our framework against three representative reconstruction paradigms:
\begin{itemize}
    \item \textit{Vanilla UBP:} A standard Universal Back-Projection assuming a constant, homogeneous SoS.
    \item \textit{Dual-SoS UBP:} An oracle baseline that utilizes the exact, ground-truth layered SoS distribution as prior knowledge for reconstruction. 
    \item \textit{Vanilla SlingBAG:} The original optimization-based method utilizing the 10-sphere approximation, without the joint ASoS field optimization.
\end{itemize}

\textbf{Evaluation Metrics.} For the \textit{in silico} experiments where the ground-truth initial pressure is available, we quantify the reconstruction fidelity using Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity Index (SSIM).

% ==========================================
\subsection{In Silico Evaluation}
\label{subsec:exp_insilico}

We first validate the theoretical superiority of our joint optimization framework on the \textit{in silico} datasets. 

%%% 在这里写一段定性分析 (Qualitative)：指出 Vanilla UBP 和 SlingBAG 会产生严重的模糊和结构错位，而你们的方法完美还原了细节，视觉效果甚至逼近开了“上帝视角”的 Dual-SoS UBP。 %%%

\begin{figure}[htbp]
    \centering
    % \includegraphics[width=\linewidth]{figs/fig_insilico_results.pdf}
    \caption{Qualitative comparison of reconstruction results on the \textit{in silico} dataset. Our method effectively eliminates acoustic aberration artifacts caused by heterogeneous SoS, achieving visual fidelity comparable to the oracle Dual-SoS UBP.}
    \label{fig:insilico_results}
\end{figure}

%%% 在这里写一段定量分析 (Quantitative)：引用下面的 Table 1，说明你们在 PSNR 和 SSIM 上取得了最高的得分（除 Oracle 外）。如果有空间，提一句你们连声速场 (ASoS Field) 都准确重建出来了。 %%%

% \begin{table}[htbp]
%     \centering
%     \caption{Quantitative evaluation (PSNR/SSIM) on the \textit{in silico} dataset.}
%     \label{tab:insilico_metrics}
%     \begin{tabular}{lcc}
%         \toprule
%         Method & PSNR $\uparrow$ & SSIM $\uparrow$ \\
%         \midrule
%         Vanilla UBP & XX.XX & 0.XXXX \\
%         Vanilla SlingBAG & XX.XX & 0.XXXX \\
%         \textbf{Ours (Auto-SoS)} & \textbf{XX.XX} & \textbf{0.XXXX} \\
%         \midrule
%         \textit{Dual-SoS UBP (Oracle)} & \textit{XX.XX} & \textit{0.XXXX} \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% ==========================================
\subsection{Experimental Validation on Physical Phantoms}
\label{subsec:exp_physical}

To demonstrate the practical applicability of our method in real-world scenarios affected by hardware noise and physical uncertainties, we evaluate it on the physical phantom dataset.

%%% 写定性分析：指出真实组织没有绝对的 GT，但从图像的锐度 (Sharpness)、对比度 (Contrast) 和边缘聚集程度来看，我们的方法在盲解 (Blind) 情况下成功校正了像差，清除了常规方法带来的伪影。 %%%

\begin{figure}[htbp]
    \centering
    % \includegraphics[width=\linewidth]{figs/fig_physical_results.pdf}
    \caption{Reconstruction results on real-world physical phantoms with complex acoustic environments. Our framework blindly resolves the acoustic aberrations, yielding significantly sharper structural boundaries compared to the baselines.}
    \label{fig:physical_results}
\end{figure}

% ==========================================
\subsection{Robustness under Sparse Sampling}
\label{subsec:exp_sparse}

In many clinical applications, dense transducer arrays are unfeasible. To evaluate the robustness of our method against ill-posed conditions, we conducted experiments under a highly sparse-view setting (e.g., retaining only 10\% of the full-view measurements).

%%% 写分析：指出基于分析的 UBP (即使是给定了精确声速的 Dual-SoS UBP) 在极度稀疏采样下也会崩溃，产生强烈的条纹伪影 (streak artifacts)。而我们的联合优化框架自带物理前向模型的约束，展现出了极强的抗混叠 (anti-aliasing) 能力。 %%%

\begin{figure}[htbp]
    \centering
    % \includegraphics[width=\linewidth]{figs/fig_sparse_results.pdf}
    \caption{Reconstruction performance under sparse-view sampling (10\% measurements). Analytical methods suffer from severe streak artifacts, whereas our optimization-based framework maintains high structural integrity.}
    \label{fig:sparse_results}
\end{figure}

% ==========================================
\subsection{Ablation Study and Efficiency Analysis}
\label{subsec:exp_ablation}

Finally, we isolate the contribution of our analytical acoustic forward model (Section 3.4) by comparing it directly against the 10-sphere approximation used in SlingBAG. 

%%% 效率分析 (Efficiency)：强调把计算复杂的 \operatorname{erf} 换成轻量级的 \exp 后，跑完一个 epoch 需要的时间大幅减少，显存 (VRAM) 占用也显著降低。 %%%

%%% 精度与收敛性分析 (Accuracy/Convergence)：指出由于解析解消除了离散近似带来的阶梯伪影，它提供了更连续的梯度流 (smoother gradient flow)，从而在优化早期实现了更稳定的收敛路径。 %%%

\begin{table}[htbp]
    \centering
    \caption{Computational efficiency analysis: Comparing the multi-sphere approximation vs. our analytical closed-form solution.}
    \label{tab:efficiency}
    \begin{tabular}{lcc}
        \toprule
        Forward Model & Time per Iteration (s) $\downarrow$ & Peak VRAM (GB) $\downarrow$ \\
        \midrule
        10-Sphere (SlingBAG) & XX.X & XX.X \\
        \textbf{Ours (Analytical)} & \textbf{X.X} & \textbf{X.X} \\
        \bottomrule
    \end{tabular}
\end{table}


==> tex/method_old.tex <==
\section{Method}

\subsection{Preliminaries}

\subsubsection{Basics of Photoacoustic Tomography}
The physical genesis of the photoacoustic tomography (PACT) signal lies in the photoacoustic effect. When a region of interest is irradiated by nanosecond pulsed laser light, specific endogenous chromophores (e.g., hemoglobin, melanin) absorb the optical energy. Under the condition of thermal confinement, this localized energy deposition translates into a rapid temperature rise and subsequent thermoelastic expansion, which excites broadband ultrasonic waves. The initial acoustic pressure, denoted as $p_0(\mathbf{r})$, propagates outward through the biological medium and is eventually captured by an array of ultrasonic transducers. The core objective of PACT reconstruction is a mathematical inverse problem: utilizing these measured, time-resolved boundary signals to recover the spatial distribution of the initial pressure $p_0(\mathbf{r})$, which serves as a proxy for the tissue's optical absorption profile. 
%
Mathematically, solving this inverse problem requires inverting the photoacoustic wave equation to back-project the received boundary signals to their spatial origins. The accuracy of this back-projection relies critically on precise acoustic time-of-flight (ToF) calculations, which are jointly determined by the relative spatial positions of the source origins and the transducer array, as well as the spatial distribution of the speed of sound (SoS) within the medium. Under ideal, simplified conditions, the medium is assumed to have a spatially uniform SoS.
%
However, real-world biological environments are inherently heterogeneous. A propagating acoustic wavefront must traverse multiple anatomical layers, such as skin, adipose tissue, muscle, and bone, each characterized by distinct sound speeds. Failure to account for these heterogeneous properties inevitably leads to severe ToF calculation errors, manifesting as defocusing artifacts and phase aberrations in the reconstructed images.

\subsubsection{3D Gaussian Splatting and SlingBAG}
Recent advancements in 3D Gaussian Splatting (3DGS) revolutionize volumetric representation and reconstruction by enabling highly efficient, fully differentiable rendering of complex 3D spatial scenes. Building upon this paradigm, the sliding Gaussian ball adaptive growth (SlingBAG) algorithm is proposed for 3D photoacoustic reconstruction. It discretizes the continuous optical absorption medium into a set of learnable, Gaussian-distributed photoacoustic sources. This explicit sparse representation provides significantly higher computational efficiency compared to traditional dense voxel grids.

To construct a fully differentiable acoustic forward model, SlingBAG must bridge explicit Gaussian-based photoacoustic source representation with wave propagation physics. However, analytically mapping a 3D Gaussian source to a time-domain transducer signal lacks a straightforward closed-form solution. To address this, SlingBAG approximates a single photoacoustic Gaussian source using a linear superposition of 10 concentric uniform spheres with varying radii $a_0^i$ and pressure amplitudes $p_0^i$. Furthermore, the standard analytical solution for a uniform solid sphere involves a non-differentiable Heaviside step function at its boundary, which fundamentally prevents gradient-based optimization. To ensure smooth backpropagation, SlingBAG replaces this sharp boundary with a differentiable approximation, $u_{\varepsilon}$, based on the error function ($\operatorname{erf}$). For a given Gaussian kernel with an effective standard deviation $\sigma = a_0$ and initial peak pressure $p_0$, its contribution to the acoustic pressure at distance $R$ and time $t$ is formulated as:
\begin{equation}
\begin{aligned}
p(R,t) &= \sum_{i=1}^{10} p_0^i \frac{D}{2R}\Big( u_{\varepsilon}(D+a_0^i) - u_{\varepsilon}(D-a_0^i) \Big), \\
\text{where} \quad D &= R-v_s t, \\
u_{\varepsilon}(x) &= \frac{1}{2}\big(1+\operatorname{erf}(\varepsilon x)\big).
\end{aligned}
\end{equation}
Here, $v_s$ represents the globally uniform speed of sound (SoS) assumed throughout the propagation medium. By linearly superimposing the pressure signals from all Gaussian photoacoustic sources, the system synthesizes the total acoustic signal received by the transducer array. Based on this differentiable forward projection, the parameters of the photoacoustic sources are iteratively optimized by minimizing the loss between the simulated and measured acoustic signals. Similar to standard 3DGS, it employs an adaptive density control mechanism: splitting regions with large gradients to capture high-frequency details and pruning negligible spheres to maintain sparsity.

While SlingBAG successfully introduces explicit sparse representations to PACT, its practical application is fundamentally limited by two critical points. First, the globally uniform SoS ($v_s$) assumption prevents it from adapting to complex tissue heterogeneities, causing phase aberrations and image defocusing. Second, approximating a continuous Gaussian kernel with 10 discrete concentric spheres imposes a severe computational burden. These underlying issues highlight the pressing need to rethink the explicit representation of both the photoacoustic sources and the acoustic medium.

% More importantly, because acoustic waves emitted from a single deep-tissue source must travel along diverse physical paths to reach different spatial locations on the transducer array, the effective SoS is not merely spatially varying, but highly anisotropic (i.e., direction-dependent). 

% \textbf{Basics of Photoacoustic Tomography (PACT):} The physical process of photoacoustic imaging begins with the illumination of biological tissue by short-pulsed laser light. Upon absorbing the pulsed optical energy, the tissue undergoes instantaneous thermoelastic expansion, which in turn excites outward-propagating ultrasonic waves, referred to as photoacoustic (PA) signals. In a PACT experiment, an ultrasonic transducer array arranged around the tissue records the time-series acoustic pressure signals throughout the propagation process. The core task of PACT reconstruction is to use these measured boundary signals to recover the initial internal pressure distribution (i.e., the source distribution) through mathematical inversion, thereby reflecting the optical absorption characteristics of the tissue. Under ideal conditions, acoustic wave propagation follows the wave equation, whose analytical solution is closely related to the spatial distribution of the speed of sound (SoS).

% \textbf{SlingBAG:} The SlingBAG algorithm discretizes continuous optical absorption sources into a set of learnable Gaussian-distributed spherical acoustic sources. This Gaussian-based sparse representation offers significantly higher computational efficiency compared to dense calculations in traditional voxel grids. In the specific implementation of SlingBAG, a constant sound speed $v_s$ is assumed throughout the space. For an ideal uniform spherical source, the generated acoustic pressure has a closed-form analytical solution. To simulate an isotropic Gaussian kernel source, SlingBAG employs a linear superposition of 10 concentric uniform spheres with different radii $a_0^i$ and pressure amplitudes $p_0^i$. To ensure gradient differentiability, it replaces the non-differentiable Heaviside step function in the physical model with a smooth approximation $u_{\varepsilon}$ based on the error function ($\operatorname{erf}$). For a Gaussian kernel with standard deviation $\sigma = a_0$ and initial peak pressure $p_0$, its contribution to the acoustic pressure at a distance $R$ and time $t$ is calculated as:
% \begin{equation}
% \begin{aligned}
% & p(R,t)=\sum_{i=1}^{10} p_0^i \frac{D}{2R}\big(
%     u_{\varepsilon}(D+a_0^i)-u_{\varepsilon}(D-a_0^i)
% \big)\\
% \text{where }& D=R-v_s t,\ u_{\varepsilon}(x)=\frac{1}{2}(1+\operatorname{erf}(\varepsilon x))
% \end{aligned}
% \end{equation}
% Based on this formula, SlingBAG linearly superimposes signals generated by all Gaussian sources and iteratively optimizes the parameters of the Gaussian kernels by minimizing the $L_2$ loss function between simulated and measured signals. Furthermore, the algorithm includes an adaptive management mechanism that splits larger spheres to capture details and prunes spheres with negligible contributions to maintain sparsity, based on the volume and contribution of the Gaussian spheres.

% \textbf{Existing Limitations:} Although SlingBAG provides an efficient reconstruction framework, its limitations remain significant. First, it assumes a completely uniform spatial SoS, which prevents it from correcting for time-of-flight deviations in heterogeneous biological tissues, leading to image aberrations. Second, the use of 10 concentric spheres to approximate a Gaussian kernel, while intuitive, leaves room for improvement in both computational efficiency (requiring 20 calls to the complex $\operatorname{erf}$ function) and accuracy (errors introduced by the approximation). To address these two bottlenecks, we propose the following improvements: first, the introduction of "Sound Speed SH Probes" as an efficient representation and optimization scheme for heterogeneous SoS fields; and second, the derivation of a more accurate and computationally faster analytical formula for Gaussian kernel signals.

%第一subsection最后的当前缺点写少点，将我们的改进和主要pipeline组合成一个新的subsection放在这里。我们的pipeline和slingBAG大致相同，主要改进为声速的计算、信号的计算（引用下文）。

\subsection{Overall Reconstruction Pipeline}
To overcome these challenges, we propose PAGS, a fully automated framework to autofocus PAT via sound-speed-adaptive Gaussian splatting. The cornerstone of our approach is a learnable, anisotropic volumetric SoS grid designed to explicitly accommodate complex tissue heterogeneities. Coupling this anisotropic SOS grid with an analytical Gaussian photoacoustic source model, our method enables the highly efficient joint optimization of both the photoacoustic sources and the acoustic medium.

The remainder of this section is organized as follows:
First, we detail the anisotropic SoS field in Sec.~\ref{sec:sos_field} . XXXX

% In Section 3.5, we derive the physics-informed forward acoustic projection that bridges these hybrid representations. Finally, the joint optimization strategy and loss functions are described in Section 3.6.

% To overcome these challenges, we propose PAGS, a fully automated framework to autofocus PAT via sound-speed-adaptive Gaussian splatting. By rigorously coupling an analytical Gaussian photoacoustic source model with a learnable, anisotropic volumetric SoS grid, our method completely eliminates discrete approximations and enables the highly efficient joint optimization of both the photoacoustic sources and the heterogeneous acoustic medium. XXX

% To accurately model the heterogeneous acoustic medium without incurring the prohibitive computational overhead of dense numerical integration, we propose a continuous, learnable 5D spatio-angular field. This field explicitly captures the anisotropic nature of acoustic wave propagation in complex tissues while maintaining a highly efficient memory footprint.


\subsection{Anisotropic Path-Averaged Speed-of-Sound Field}
\label{sec:sos_field}

\subsubsection{From Explicit Medium Segmentation to Implicit Time-of-Flight Modeling}

To account for an inhomogeneous SoS medium, conventional reconstruction methods (e.g., multi-SoS universal back-projection) attempt to explicitly model the physical spatial layout of the acoustic medium. They typically partition the imaging region into discrete segments and assign different average speeds to each anatomical structure. However, this explicit medium modeling relies heavily on strong anatomical priors (e.g., explicit tissue segmentation from other modalities) and fundamentally lacks the flexibility for end-to-end optimization. Furthermore, calculating the exact wave propagation under this paradigm requires complex ray-region intersection tests and dense path integration computation, which is computationally intractable for iterative joint optimization.

Returning to the first principles of PACT, we recognize a critical disconnect in traditional approaches: back-projection focusing algorithms do not inherently require the precise spatial boundaries or internal distribution of different tissues. Instead, the core physical variable that governs the focusing quality is solely the macroscopic acoustic time-of-flight (ToF) between the photoacoustic source and the transducer. 
%
Based on this insight, we propose a shift from explicit medium segmentation to implicit ToF modeling. We completely bypass the necessity of segmenting the physical medium and directly capture the cumulative ToF effect through a continuous spatio-angular field. Physically, the average sound speed along a propagation path inherently varies depending on both the source's spatial location $\mathbf{x}$ and the emission direction $\boldsymbol{\omega}$ toward a specific transducer. Crucially, because biological tissues are typically piecewise smooth and the transducer array is distributed on a continuous convex manifold, this path-averaged SoS exhibits a low-frequency, continuous distribution across both spatial and angular domains. 

This intrinsic smoothness allows us to elegantly compress the computationally prohibitive dense path integration into a 5D \textbf{anisotropic path-averaged speed of sound (ASoS) field}. Consequently, for a given Gaussian photoacoustic source located at $\mathbf{x}$ and a transducer at $\mathbf{z}$, we can concisely model the ToF as:
\begin{equation}
% \begin{center}
\text{ToF}(\mathbf{x}, \mathbf{z}) = \frac{\lVert\mathbf{z} - \mathbf{x}\rVert}{v_{avg}(\mathbf{x}, \boldsymbol{\omega})},
% \end{center}    
\end{equation}
where $\boldsymbol{\omega} = (\mathbf{z} - \mathbf{x}) / \lVert\mathbf{z} - \mathbf{x}\rVert$ is the normalized direction vector, and $v_{avg}(\mathbf{x}, \boldsymbol{\omega})$ is the evaluated path-averaged SoS from our continuous 5D field.

\subsubsection{Anisotropic SoS Field Parameterization via Spherical Harmonic Probes}
To transform the continuous 5D ASoS field into a highly expressive and trainable form, we introduce the concept of \textbf{Sound Speed Spherical Harmonic Probes}. In standard 3D Gaussian Splatting architectures, view-dependent properties (like color) are typically modeled by assigning independent SH coefficients directly to each discrete Gaussian primitives. However, adopting this naive paradigm for the sound speed modeling is physically problematic. Because discrete Gaussians lack inherent topological connectivity, assigning independent SoS coefficients to them would destroy the spatial continuity of the acoustic field. Enforcing smoothness on such an unstructured point cloud would necessitate computationally prohibitive neighborhood queries (e.g., K-Nearest Neighbors) at every iteration.

To intrinsically enforce spatial smoothness without sacrificing efficiency, we decouple the acoustic medium from the individual Gaussian photoacoustic sources. We divide the imaging region into a 3D volumetric grid and anchor an SH probe at each voxel center. Inspired by irradiance probes in global illumination, each probe encodes the angular distribution of the path-averaged SoS at its specific spatial location. 
%
To mathematically parameterize this angular dependence, we utilize orthogonal Spherical Harmonic (SH) basis functions. For a given SH degree $D$, the SH basis evaluated at any target direction $\boldsymbol{\omega}$ is simply expressed as a basis vector $\mathbf{Y}(\boldsymbol{\omega}) \in \mathbb{R}^{K_{sh}}$, where $K_{sh} = (D+1)^2$. 
%
Correspondingly, each probe stores a learnable coefficient vector $\mathbf{c} \in \mathbb{R}^{K_{sh}}$ that serves as the specific weights for this basis. The continuous angular SoS distribution at the probe's location is then formulated as a linear combination, concisely expressed as a vector dot product:
\begin{equation}
    v_{avg}(\boldsymbol{\omega}) = \mathbf{c} \cdot \mathbf{Y}(\boldsymbol{\omega})
\end{equation}
where the coefficients $\mathbf{c}$ effectively modulate the acoustic anisotropy.
%
By extracting the local SH coefficients through spatial interpolation of the adjacent bounding probes, any dynamic photoacoustic source located at an arbitrary position $\mathbf{x}$ can continuously query the ASoS. Crucially, this grid-based anchoring acts as a \textbf{structural regularizer}: the inherent interpolation naturally constrains the spatial smoothness of the SoS field, completely bypassing the need for explicit, expensive neighborhood constraints.

\subsubsection{Memory-Efficient ASoS Field Interpolation}
To reconstruct the photoacoustic sources, we must evaluate the path-averaged SoS $v_{avg}(\mathbf{x}, \boldsymbol{\omega})$ for every source-to-transducer pair. This requires querying the static SH probes from the continuous positions of dynamic Gaussian kernels. 

For any photoacoustic source at $\mathbf{x}$, its local acoustic properties are determined by the eight surrounding probes in the volumetric grid. We define $w_{i,j,k}(\mathbf{x})$ as the standard trilinear interpolation weights derived from the relative displacement between $\mathbf{x}$ and the probe positions. 
%
Given these interpolation weights, the most intuitive computational path (the \textbf{angular-then-spatial} strategy) is to first resolve the angular dependency at each grid node. Mathematically, this corresponds to:
\begin{equation}
    v_{avg}(\mathbf{x}, \boldsymbol{\omega}) = \sum_{i,j,k} \left( \mathbf{c}_{i,j,k} \cdot \mathbf{Y}(\boldsymbol{\omega}) \right) w_{i,j,k}(\mathbf{x})
\end{equation}
However, this sequence is practically prohibitive for high-resolution PACT. Computing the terms inside the parentheses first necessitates caching a massive intermediate tensor of size $\mathcal{O}(N_{probe} \times N_{transducer})$. In our setup ($N_{probe} \approx 64^3$, $N_{transducer} \approx 4000$), this intermediate representation consumes dozens of gigabytes of VRAM, triggering catastrophic Out-Of-Memory (OOM) failures during gradient caching.

To resolve this bottleneck, we exploit the associative property of linear combinations to invert the computational order, proposing a \textbf{spatial-then-angular} interpolation strategy:
\begin{equation}
    v_{avg}(\mathbf{x}, \boldsymbol{\omega}) = \left( \sum_{i,j,k} \mathbf{c}_{i,j,k} w_{i,j,k}(\mathbf{x}) \right) \cdot \mathbf{Y}(\boldsymbol{\omega})
\end{equation}
By executing the spatial interpolation (inside the parentheses) first, we restrict the peak intermediate tensor size to merely $\mathcal{O}(N_{gaussian} \times K_{sh})$, where $K_{sh} = 9$ for 2-order SH functions and 
$N_{gaussian} \approx XXX$.
%
This permutation reduces the GPU memory cost by orders of magnitude. This strategy ensures the scalable joint optimization of massive Gaussian kernels coupled with a dense, anisotropic acoustic medium on standard consumer-grade GPUs.


% \subsection{XXX}
% %这里加少量内容表示下面要做什么。

% \textbf{Fundamental Assumptions:} To handle heterogeneous sound speeds with controllable computational overhead, we establish a set of physical approximations. We assume that while the spatial SoS distribution fluctuates, it is locally smooth and slowly varying. Under this premise, we ignore severe ray bending (refraction) and complex wavefront distortions, focusing instead on the cumulative effect of SoS variations on the arrival time at the transducers. Consequently, for the signal generated by any Gaussian kernel at a given transducer, we replace the uniform $v_s$ in the formula with the \textbf{average speed of sound} along the straight-line path from the Gaussian kernel to the transducer. However, assigning an independent SoS parameter to every "Gaussian-transducer" pair would lead to a parameter scale of $O(N_{gaussian} \times N_{transducer})$, which is unacceptable in terms of memory and computation. Moreover, since Gaussian kernels move dynamically during optimization, binding SoS directly to the kernels would lead to a lack of spatial consistency in adjacent regions. Thus, we propose a static average SoS field that compresses parameters through sampling and Spherical Harmonic (SH) approximation.

% %下一段加少量内容表示提出声速场的用意（一次插值得到平均声速）。

% \textbf{Average Speed of Sound Field:} We define a five-dimensional continuous Average Speed of Sound (AvgSoS) field. In a PACT system, all transducers are distributed on the surface $S$ of a 3D convex volume $V$ enclosing the reconstruction region. For any point $\vec{x}$ inside the volume (a potential Gaussian kernel location) and any unit direction vector $\vec{d} \in \mathbb{S}^2$, a ray starting from $\vec{x}$ along $\vec{d}$ intersects the surface $S$ at a unique detection point $\vec{z}$. The AvgSoS field is defined as the function $\text{AvgSoS}(\vec{x},\vec{d}) = v_{x-z}$, where $v_{x-z}$ is the average SoS along the path $\vec{x} \to \vec{z}$. This definition naturally extends complex path integration properties to the entire space. Given the slow variation of SoS in tissue, this field is a smooth continuous function of both position $\vec{x}$ and direction $\vec{d}$. Despite being 5D, its low-frequency nature allows for high-precision approximation with few parameters.

% \textbf{Sound Speed Probes:} To make the AvgSoS field trainable and parametric, we introduce the concept of "Sound Speed SH Probes." We divide the 3D reconstruction space into a uniform grid and place a probe at each grid node $\vec{p}_{i,j,k}$. Each probe stores the angular AvgSoS distribution function at that location. Inspired by Spherical Harmonic Lighting in computer graphics, we utilize the first $k$ orders of SH functions as an orthogonal basis to expand and approximate the angular function $\text{AvgSos}_{\vec{x}_0}(\vec{d})$. Each probe only needs to store $k^2$ SH coefficients $\vec{c}_{i,j,k}$. This representation is highly compact; it not only stores local SoS characteristics but also ensures global spatial continuity through the grid layout. By optimizing these coefficients, we can learn a heterogeneous SoS model that is both physically consistent and highly expressive.

% \textbf{Field Interpolation:} In each epoch of the reconstruction process, we must compute the average SoS from every dynamic Gaussian kernel to every transducer. To minimize computational overhead and memory footprint, we implement a two-stage interpolation strategy: first, spatial interpolation of the SH coefficients, followed by angular interpolation to obtain the scalar SoS. While the order of these operations can be mathematically swapped with an identical result, our "spatial-then-angular" sequence significantly reduces the size of intermediate tensors.

% Specifically, for a Gaussian kernel located at $\vec{x}$ and a transducer at $\vec{z}$:
% \begin{enumerate}
%     \item \textbf{Spatial Interpolation:} We first perform trilinear interpolation to extract the SH coefficients $\vec{c}$ at position $\vec{x}$ from the coefficients $\vec{c}_{i,j,k}$ of the 8 surrounding probes. Let $l$ be the grid spacing and $\vec{p}_{i,j,k}$ be the probe positions. We denote the relative displacement as $\vec{x} - \vec{p}_{i,j,k} = (\Delta x, \Delta y, \Delta z)$. The trilinear interpolation weight $w_{i,j,k}$ for each probe is then calculated as:
%     $$
%     w_{i,j,k}=\max\{0,1-\lvert\Delta x\rvert/l\}\max\{0,1-\lvert\Delta y\rvert/l\}\max\{0,1-\lvert\Delta z\rvert/l\}$$
%     The interpolated coefficient vector is $\vec{c}=\sum_{i,j,k}\vec{c}_{i,j,k}w_{i,j,k}$.
    
%     \item \textbf{Angular Interpolation:} Given the local coefficients $\vec{c}$, we calculate the normalized direction vector $\vec{d}=(\vec{z}-\vec{x})/\lVert\vec{z}-\vec{x}\rVert$. The average SoS is then calculated by the dot product with the SH basis $\vec{Y}(\vec{d})$:
%     $$v_{x-z}=\vec{c}\cdot\vec{Y}(\vec{d})$$
% \end{enumerate}

% As shown in the following equation, the linearity of the dot product ensures that performing spatial interpolation before angular interpolation is mathematically equivalent to the reverse:
% \begin{equation}
% \vec{c} \cdot \vec{Y}(\vec{d}) = \bigg( \sum_{i,j,k} \vec{c}_{i,j,k} w_{i,j,k} \bigg) \cdot \vec{Y}(\vec{d}) = \sum_{i,j,k} \left( \vec{c}_{i,j,k} \cdot \vec{Y}(\vec{d}) \right) w_{i,j,k}
% \end{equation}

% However, the computational efficiency differs vastly. If we were to perform angular interpolation first, we would need to compute the SoS for every probe-transducer pair, resulting in an intermediate representation of size $O(N_{probe} \times N_{transducer})$. In contrast, our proposed order only requires storing the interpolated SH coefficients for each Gaussian kernel, resulting in an intermediate size of $O(N_{gaussian} \times k^2)$. Since the SH order $k$ is small (e.g., $k=3$), $N_{gaussian}k^2$ is much smaller than $N_{probe}N_{transducer}$ in typical PACT setups. This strategy drastically reduces GPU memory consumption, enabling the simultaneous optimization of a large number of Gaussian kernels and the SoS field.

\subsection{Analytical Acoustic Forward Model}
Once the anisotropic SoS field is evaluated, the subsequent step is performing the forward acoustic projection to the transducer array. However, the existing multi-sphere approximation in SlingBAG relies on multiple costly error function ($\operatorname{erf}$) evaluations, creating a computational bottleneck during optimization.
%
To address this bottleneck, we derive an approximate closed-form solution based on the 3D acoustic wave equation. For a Gaussian photoacoustic source with initial pressure $p_0(\mathbf{r}) = p_0 \exp(-\|\mathbf{r}\|^2 / 2\sigma^2)$, the exact closed-form solution in an ideal medium is:
\begin{equation}
\begin{aligned}
p(R, t) &= \frac{p_0}{2R} (R - v_s t) \exp\left( -\frac{(R - v_s t)^2}{2\sigma^2} \right) \\
&+ \frac{p_0}{2R} (R + v_s t) \exp\left( -\frac{(R + v_s t)^2}{2\sigma^2} \right),
\end{aligned}
\end{equation}
where $v_s$ is the speed of sound, $R$ is the observation distance, and $\mathbf{r}$ denotes the spatial coordinate relative to the Gaussian center.

Physically, the first term represents an outgoing acoustic wave, while the second term represents an incoming converging wave. At the effective time of acoustic detection ($t \approx R/v_s$), the exponential envelope of the second term evaluates to $\exp(-2R^2/\sigma^2)$. Because PACT transducers are typically located in the far-field relative to the imaging target ($R \gg \sigma$), this incoming wave term decays to zero. By discarding this vanishing term and substituting the constant $v_s$ with our interpolated ASoS field $v_{avg}(\mathbf{x}, \boldsymbol{\omega})$, we obtain a streamlined far-field asymptotic solution:
\begin{equation}
p(R, t) \approx \frac{p_0 (R - v_{avg}0t)}{2R} \exp\left( -\frac{(R - v_{avg}t)^2}{2\sigma^2} \right)
\end{equation}

Compared to the multi-sphere approximation, this analytical formulation theoretically offers advantages in both accuracy and efficiency. The accuracy is ensured by the rigorous analytical derivation under the highly valid far-field assumption, while the computational speedup is naturally achieved by replacing complex numerical fittings with a concise closed-form evaluation. These performance gains are empirically demonstrated in Section \ref{sec:experiments}.

\subsection{Joint Optimization and Loss Formulation}

With the differentiable analytical forward model established, we frame the PACT reconstruction as a joint optimization problem. Our goal is to simultaneously recover the photoacoustic source parameters (i.e., positions $\mathbf{x}$, amplitudes $p_0$, and scales $\sigma$ of the Gaussian kernels) and the heterogeneous acoustic medium (i.e., the SH coefficients $\mathbf{c}$ of the volumetric grid).

For a given transducer located at $\mathbf{z}_m$, the total projected pressure signal $\hat{p}(\mathbf{z}_m, t)$ is the linear superposition of the analytical waveforms generated by all $N$ Gaussian sources:
\begin{equation}
    XXX
\end{equation}
XXX. 

To drive the optimization, we minimize the discrepancy between the projected signals $\hat{p}$ and the ground-truth measurements $p_{gt}$ captured by the transducer array. We employ XXXX:
\begin{equation}
    XXXX
\end{equation}
Depending on the complexity of the acoustic environment, an optional spatial regularization term $\mathcal{R}_{TV}(\mathbf{c})$ (e.g., Total Variation) can be applied to the SH grid to further encourage macroscopic smoothness in the reconstructed ASoS field. 

% \subsection{Signal Computation}

% After calculating the precise path-average SoS, efficiently converting it into pressure signals is crucial. The 10-sphere approximation used in SlingBAG is mathematically imprecise, computationally expensive (20 $\operatorname{erf}$ calls), and introduces non-physical high-frequency "staircase" artifacts due to its discrete nature. These artifacts introduce gradient noise during backpropagation, hindering convergence and degrading image quality.

% To improve accuracy and stability, we derive an analytical solution for the Gaussian kernel based on the Poisson formula of the wave equation. For an initial pressure distribution $p_0(\vec{r}) = p_0 \exp(-\|\vec{r}\|^2 / 2\sigma^2)$, the exact closed-form solution in an ideal medium is:
% \begin{equation}
% p(R, t) = \frac{p_0}{2R} (R - v_s t) \exp\left( -\frac{(R - v_s t)^2}{2\sigma^2} \right) + \frac{p_0}{2R} (R + v_s t) \exp\left( -\frac{(R + v_s t)^2}{2\sigma^2} \right)
% \end{equation}
% This solution consists of an outgoing wave and an incoming wave that passes through the center. The second term decays exponentially as the observation distance $R$ increases. In PACT, transducers are typically located far from the tissue (far-field condition, $R \gg \sigma$). By discarding the decaying term, we obtain a streamlined far-field asymptotic solution:
% \begin{equation}
% p(R, t) \approx \frac{p_0 (R - v_s t)}{2R} \exp\left( -\frac{(R - v_s t)^2}{2\sigma^2} \right)
% \end{equation}
% We substitute the average SoS $v_{x-z}$ obtained from the SH probes for $v_s$ in this formula.

% Compared to the multi-sphere approximation, our analytical formula provides a perfectly smooth and physically continuous waveform, eliminating discretization artifacts. As the analytical solution is highly differentiable, it provides more stable gradient flows, preventing the optimization from trapping in local optima. Furthermore, the new formula simplifies complex function calls into a single $\exp$ operation, resulting in a multi-fold speedup in GPU parallel computing.

% By integrating the Sound Speed SH Probes with the optimized analytical signal model, we have constructed a new PACT reconstruction framework capable of handling complex acoustic environments with high computational efficiency.

==> tex/relatedwork_old.tex <==
\section{Related Work}
\label{sec:related}
\subsection{PACT Reconstruction Methods}
Conventional PACT reconstruction algorithms are broadly categorized into analytical and iterative paradigms. Analytical methods, predominantly Universal Back-Projection (UBP)~\cite{xu2005universal} and Delay-and-Sum (DAS), are widely adopted for their computational efficiency. By deterministically mapping time-resolved signals to the spatial domain, they operate on the highly idealized assumption of straight-ray propagation within a homogeneous medium. However, this assumption critically fails in realistic biological tissues~\cite{lin2025survey,poimala2024compensating}. Acoustic heterogeneities across diverse tissue layers induce wavefront refraction and significant time-of-flight (ToF) mismatches. Since manual global SoS tuning cannot compensate for these localized phase errors, analytical reconstructions inherently suffer from geometric distortions, spatial blurring, and severe resolution degradation~\cite{yang2025skull}. Furthermore, these methods strictly rely on dense spatial sampling to guarantee reconstruction fidelity. Under sparse sensor coverage or limited-view geometries, they lack the inherent mechanisms to constrain the solution space, inevitably generating streak artifacts and making reliable structure identification exceedingly difficult~\cite{li2024slingbag,lin2025survey}.

To address these limitations, model-based iterative reconstruction methods formulate PACT as an optimization-driven inverse problem \xiaoyun{add more references here, refer Prof. Mark Anastasio's work in UIUC}. By integrating regularization terms such as Total Variation (TV) or $L_1$-norm penalties, these frameworks achieve superior resilience against sparse sampling and measurement noise. However, the repeated evaluation of the forward acoustic propagation and its adjoint gradient inherently incurs substantial computational and memory costs. Furthermore, standard iterative frameworks typically rely on a predefined SoS map for accurate forward modeling. In realistic biological tissues, acquiring the exact anatomical SoS distribution is highly challenging. Inaccuracies in this static prior can compromise the compensation of acoustic aberrations, ultimately limiting the overall reconstruction fidelity~\cite{song2023sparse}.

In recent years, deep learning has emerged as a powerful alternative for PACT reconstruction. Data-driven architectures, ranging from U-Nets to diffusion models, leverage rich learned priors to achieve striking artifact reduction under ill-posed conditions, such as sparse-view or limited-aperture scenarios~\cite{song2023sparse,liu2024recent,lin2025survey}. While these purely data-driven networks offer impressive structural restoration, pioneering physics-aware frameworks have further attempted to explicitly incorporate physical constraints to dynamically resolve unknown acoustic aberrations. For instance, Poimala \textit{et al.} designed a specialized network to compensate for unknown SoS distributions, effectively recovering spatial resolution degraded by wavefront aberrations~\cite{poimala2024compensating}. Similarly, Li \textit{et al.} employed coordinate-based implicit neural representations to directly recover a spatial SoS field jointly with the absorption distribution, enabling aberration correction through physically informed decoding~\cite{li2025coordinate}. Together, these learning-based and physics-aware approaches demonstrate the immense potential of integrating data-driven priors with acoustic physical models. However, despite their success in accounting for non-uniform SoS, representing the acoustic field via dense grids or implicit functions remains computationally demanding, limiting their scalability and memory efficiency in complex 3D environments.

\subsection{Gaussian-based Reconstruction Methods}

3D Gaussian Splatting (3DGS)~\cite{kerbl20233d}\xiaoyun{add more references here} has emerged as a powerful explicit scene representation paradigm. Instead of relying on traditional voxels or meshes, it parameterizes a scene using a collection of learnable, anisotropic 3D Gaussian primitives. Each primitive is explicitly defined by its position, covariance, opacity, and view-dependent color. Rendered via a highly efficient differentiable tile-based rasterizer, 3DGS achieves real-time performance while preserving state-of-the-art visual fidelity.
%
This structural flexibility and computational efficiency have inspired a surge of dynamic extensions. For instance, Deformable 3DGS~\cite{yang2024deformable} introduces a per-Gaussian temporal deformation field, allowing the framework to reconstruct high-quality geometry and appearance from monocular dynamic videos. Building upon the concept of temporal modeling, 4DGS~\cite{wu20244d} directly embeds the optimization into the space-time domain, jointly updating Gaussian attributes and motion trajectories to enable real-time dynamic view synthesis. Furthermore, Spacetime Gaussian Feature Splatting~\cite{li2024spacetime} explicitly models the evolution of both geometry and appearance using polynomial trajectories, which significantly enhances the temporal coherence of dynamic renderings. 
%
Collectively, these advances highlight the core strengths of Gaussian-based representations. As explicit, grid-free primitives, they can efficiently capture fine geometric details, seamlessly adapt to complex topological changes, and maintain full end-to-end differentiability, establishing 3DGS as a highly expressive and robust spatial modeling framework.

Building upon this momentum, Gaussian representations have been rapidly adapted to medical tomographic reconstruction. In X-ray computed tomography (CT), $R^2$-Gaussian~\cite{zha2024r2gaussian} introduced a radiometrically corrected Gaussian splatting forward model that compensates for scattering and beam hardening effects, achieving high-quality 3D reconstructions under sparse-view acquisition. Similarly, for 3D ultrasound volume imaging, UltraGauss~\cite{eid2025ultragauss} integrated learnable Gaussian primitives with an acoustic wave propagation renderer to build a fast reconstruction framework, demonstrating strong adaptability to reflection and attenuation physics. These successful cross-modal adaptations confirm that, when equipped with modality-specific differentiable forward models, Gaussian primitives can serve as a highly expressive and versatile basis for solving complex volumetric inverse problems.

In the realm of PACT, SlingBAG~\cite{li2024slingbag} recently pioneered the integration of Gaussian representations by parameterizing the initial photoacoustic pressure as a collection of learnable 3D Gaussian PA sources. For acoustic forward projection, it approximates each continuous Gaussian primitive by multiple concentric spherical shells and uses a smoothed sphere response with error-function evaluations to maintain differentiability. While effective, this approximation increases the per-iteration computational cost and still fundamentally hinges on a globally homogeneous SoS assumption. Under this constraint, the acoustic time-of-flight from each Gaussian PA source to each detector is evaluated solely from Euclidean distance, neglecting path-dependent aberrations caused by heterogeneous acoustic media. Consequently, the uniform-SoS limitation leads to structural defocusing and geometric distortion, compromising spatial resolution and reconstruction fidelity.

These limitations motivate PAGS, an SoS-adaptive Gaussian splatting framework for blind autofocusing PACT. PAGS keeps the sparse Gaussian PA source representation, replaces the multi-sphere approximation with an analytic Gaussian acoustic projection, and introduces a learnable anisotropic path-averaged SoS field parameterized by compact spherical harmonic (SH) probes. In this way, PAGS optimizes the source representation and the path-level propagation correction directly from measured transducer signals, without recovering a dense physical SoS map.

% In recent years, deep learning has emerged as a powerful alternative for PACT reconstruction. Data-driven architectures, ranging from U-Nets to diffusion models, leverage rich learned priors to achieve striking artifact reduction under ill-posed conditions (e.g., sparse-view or limited-aperture)~\cite{song2023sparse,liu2024recent,lin2025survey}. However, purely data-driven models typically operate as black-box mappings; they implicitly assume a homogeneous medium and lack the explicit physical constraints required to resolve complex acoustic aberrations.
% To bridge this gap, pioneering physics-aware frameworks have attempted to incorporate SoS heterogeneities. For instance, Poimala \textit{et al.} designed a specialized network for aberration compensation~\cite{poimala2024compensating}, while Li \textit{et al.} employed Implicit Neural Representations (INRs) to jointly recover the SoS and absorption distributions~\cite{li2025coordinate}. Despite these promising advances, evaluating the path-integrated acoustic time-of-flight remains a fundamental bottleneck. Extracting path-averaged SoS from dense scalar grids or implicit MLPs necessitates continuous ray-marching and intensive point-wise evaluations along every acoustic ray. This process incurs prohibitive memory consumption and severely limits training efficiency. 
% Therefore, developing a compact representation that intrinsically and efficiently encodes the directional, path-dependent SoS without heavy numerical integration remains a critical challenge for clinically realistic PACT.

% \subsection{PACT Reconstruction Methods}

% Photoacoustic computed tomography (PACT) reconstructs the initial pressure distribution from acoustic signals acquired by ultrasound transducers.
% Conventional reconstruction algorithms fall into analytical and iterative categories.
% Analytical methods, most notably Universal Back‑Projection (UBP)~\cite{xu2005universal} and Delay‑and‑Sum (DAS), back‑project the measured time‑resolved pressure signals along straight acoustic ray paths.
% They are built on the idealizing assumption of a homogeneous medium with constant sound speed, which gives them low computational complexity and ease of implementation.
% However, real biological tissues—comprising fat, muscle, bone, and blood—exhibit substantially different acoustic impedances, leading to spatially varying sound speed distributions that can deviate from a global average by up to several percent~\cite{lin2025survey,poimala2024compensating}.
% When ultrasound pulses traverse these heterogeneous regions, wavefront refraction and propagation time shifts occur.
% The resulting time‑of‑flight mismatches produce geometric distortion, amplitude blurring, and diffuse structural artifacts in the reconstructed images~\cite{yang2025skull}.
% Manually tuning a global sound speed cannot compensate for localized heterogeneities, severely limiting the utility of analytical methods for realistic samples.
% Furthermore, under sparse sensor coverage, limited view angles, or restricted detection apertures, analytical back‑projection generates severe streak artifacts, trailing, and loss of fine detail, making reliable structure identification difficult~\cite{li2024slingbag,lin2025survey}.

% Iterative reconstruction approaches formulate the problem as an inverse problem, typically adding sparsity‑inducing regularization terms such as total variation or \(L_1\)‑norm penalties to suppress noise and artifacts.
% While capable of improving image quality under sparse sampling, they demand repeated forward simulations and adjoint back‑projections, incurring high computational cost and slow convergence.
% More critically, many iterative frameworks require a predefined sound speed map as a prior.
% If the prior deviates from the true distribution, the iterations may not correct but instead amplify the distortions, compromising robustness in unknown acoustic environments~\cite{song2023sparse}.

% In recent years, deep learning has opened new avenues for PACT reconstruction.
% Architectures including U‑Net, generative adversarial networks, and diffusion models have been trained on large paired datasets to learn the mapping from measurement signals to initial pressure, achieving striking artifact reduction and structural restoration under sparse‑view, limited‑aperture, or low‑dose conditions~\cite{song2023sparse,liu2024recent,lin2025survey}.
% These methods encapsulate rich anatomical priors that compensate for the lack of explicit physical regularization.
% Nevertheless, most purely data‑driven models still implicitly rely on a uniform sound speed assumption and lack an explicit mechanism to model the path‑integrated effect of acoustic propagation.
% A few pioneering works have attempted to bridge this gap: Poimala \textit{et al.} designed a specialized network to compensate for unknown sound speed distributions, recovering resolution lost to wavefront aberrations~\cite{poimala2024compensating}; Li \textit{et al.} employed a coordinate‑based neural network to directly recover a spatial sound speed field jointly with the absorption distribution, enabling aberration correction through physically informed decoding~\cite{li2025coordinate}.
% Although these methods demonstrate promising awareness of non‑uniform sound speed, representing the field as a dense volumetric grid or an implicit coordinate‑based function often incurs high memory consumption, slow training convergence, and does not naturally capture the path‑integrated nature of acoustic time‑of‑flight.
% Thus, a compact and efficient representation of path‑dependent sound speed effects remains a critical challenge for promoting PACT from idealized homogeneous assumptions to clinically realistic scenarios.

% \subsection{Gaussian-based Reconstruction Methods}

% 3D Gaussian Splatting (3D‑GS)~\cite{kerbl20233d} has emerged as a revolutionary scene representation paradigm.
% Instead of using voxels or meshes, it explicitly parameterizes a scene as a collection of learnable anisotropic 3D Gaussian primitives, each defined by a position, covariance, opacity, and view‑dependent color.
% A highly efficient differentiable tile‑based rasterizer renders these primitives, achieving real‑time performance while preserving state‑of‑the‑art visual fidelity.
% This flexibility and efficiency have inspired a surge of dynamic extensions: Deformable 3D‑GS learns a per‑Gaussian temporal deformation field to reconstruct high‑quality geometry and appearance from monocular dynamic videos~\cite{yang2024deformable}; 4D‑GS jointly optimizes Gaussian attributes and motion trajectories directly in space‑time to enable real‑time dynamic view synthesis~\cite{wu20244d}; and Spacetime Gaussian Feature Splatting encodes the geometry and appearance evolution with polynomial trajectories, further enhancing the coherence of dynamic renderings~\cite{li2024spacetime}.
% These advances collectively demonstrate that Gaussian‑based representations, as explicit point‑based primitives, possess the capacity to capture fine geometric details, adapt to topological changes, and maintain full differentiability, making them a powerful general substrate for solving complex physical inverse problems.

% Inspired by this momentum, Gaussian representations have been rapidly adapted to medical tomographic reconstruction.
% In X‑ray computed tomography, R\textsuperscript{2}-Gaussian introduced a radiometrically corrected Gaussian splatting forward model that compensates for scattering and beam hardening effects, achieving high‑quality 3D reconstruction under sparse‑view acquisition~\cite{zha2024r2gaussian}.
% For 3D ultrasound volume imaging, UltraGauss fused learnable Gaussian kernels with an acoustic wave propagation renderer to build an ultrafast reconstruction framework, demonstrating strong adaptability to reflection and attenuation physics~\cite{eid2025ultragauss}.
% These successful cross‑modal transfers confirm that, when equipped with modality‑specific differentiable physical renderers, Gaussian primitives can serve as an expressive basis for volumetric inverse problems.

% In the realm of PACT, SlingBAG (Sliding Gaussian Ball Adaptive Growth)~\cite{li2024slingbag} pioneered the use of Gaussian representations by modeling the optical absorption distribution as a set of learnable spherical Gaussian sources.
% It employs a dynamic adaptive growth strategy: large Gaussians are split based on their volume and contribution to capture finer structures, while weakly contributing sources are pruned to maintain sparsity.
% This design yields impressive reconstruction quality under sparse sampling and limited‑view conditions, significantly outperforming traditional analytical methods.
% However, SlingBAG's forward acoustic model fundamentally assumes a globally homogeneous sound speed.
% The propagation time from each Gaussian to each sensor is determined solely by geometric distance, ignoring any path‑dependent sound speed variations in heterogeneous tissues.
% When the true tissue sound speed distribution is non‑uniform, time‑of‑flight misalignments systematically shift the optimized Gaussian positions and corrupt intensity accumulation, leading to localization biases and contrast degradation.
% Thus, while the Gaussian representation offers unprecedented flexibility for PACT, the uniform sound speed constraint constitutes a major bottleneck for practical application in complex biological environments.

% To overcome this limitation, we introduce trainable spherical harmonic sound speed probes.
% Our method encodes the path‑averaged sound speed field into a compact set of low‑order spherical harmonic coefficients stored on a spatial grid.
% This representation seamlessly integrates with the Gaussian splatting framework, enabling joint optimization of the absorption parameters of Gaussian primitives and the non‑uniform sound speed distribution with negligible extra memory overhead.
% By explicitly compensating for propagation time aberrations induced by tissue heterogeneities, our framework significantly enhances the robustness and quantitative accuracy of PACT reconstruction in realistic biological media.

